Semantically Distributed Robust Optimization for Vision-and-Language Inference

Analysis of vision-and-language models has revealed their brittleness under linguistic phenomena such as paraphrasing, negation, textual entailment, and word substitutions with synonyms or antonyms. While data augmentation techniques have been designed to mitigate against these failure modes, methods that can integrate this knowledge into the training pipeline remain under-explored. In this paper, we present \textbf{SDRO}, a model-agnostic method that utilizes a set linguistic transformations in a distributed robust optimization setting, along with an ensembling technique to leverage these transformations during inference. Experiments on benchmark datasets with images (NLVR$^2$) and video (VIOLIN) demonstrate performance improvements as well as robustness to adversarial attacks. Experiments on binary VQA explore the generalizability of this method to other V\&L tasks.

==> supp_tables/violin_text_attack.tex <==
\begin{table}[t]
    \centering
    \small 
    {\resizebox{\linewidth}{!}{
    \begin{tabular}{@{}p{15mm} ccccccc@{}}
        \toprule
        % \multirow{2}{*}{\textbf{Model}} & \multicolumn{7}{c}{\textbf{Text Attack Categories}} \\
        \textbf{Model} & \textbf{CLARE} & \textbf{CharSwap} & \textbf{CheckList} & \textbf{EDA} & \textbf{Emb} & \textbf{WordNet} & \textbf{Avg.}\\
        \midrule
        HERO          & 66.08  & 63.00 & 68.58 & 60.89 & 63.81 & 63.38 & 64.29 \\
        HERO{+}SDRO   & 68.70 & 64.95 & 68.96 & 61.32 & 65.54 & 64.61 & 65.68 \\
        \bottomrule 
    \end{tabular}
    }
    }
    \caption{Performance on VIOLIN ``text-attack'' set created using augmentation techniques from Text-Attack.}
    \label{tab:violin_text_attack}
\end{table}

==> supp_tables/vqa_textattack.tex <==
\begin{table}[ht]
    \centering
    \small 
    {\resizebox{\linewidth}{!}{
    \begin{tabular}{@{}p{15mm} ccccccc@{}}
        \toprule
        % \multirow{2}{*}{\textbf{Model}} & \multicolumn{7}{c}{\textbf{Text Attack Categories}} \\
        \textbf{Model} & \textbf{CLARE} & \textbf{CharSwap} & \textbf{CheckList} & \textbf{EDA} & \textbf{Emb} & \textbf{WordNet} & \textbf{Avg.}\\
        \midrule 
        UN          & 80.82 & 75.74 & 82.46 & 72.74 & 76.94 & 76.85 & 77.59 \\
        UN + SDRO   & 83.57 & 77.72 & 84.43 & 74.05 & 80.31 & 73.38 & 78.91 \\
        \midrule 
        VI          & 80.49 & 75.74 & 84.87 & 74.64 & 78.63 & 76.39 & 78.45 \\
        VI + SDRO   & 85.99 & 84.52 & 84.10 & 87.02 & 84.25 & 84.03 & 84.99 \\
        \bottomrule
    \end{tabular}
    }
    }
    \caption{Performance on VQA-Yes/No ``text-attack'' set created using augmentation techniques from Text-Attack.}
    \label{tab:vqa_text_attack}
\end{table}

==> tables/contrast_sets.tex <==
\begin{table}[t]
    \centering
    \footnotesize
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{c cc c cc}
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c}{\textbf{Accuracy}} & \hphantom &  \multicolumn{2}{c}{\textbf{Consistency}} \\
        \cmidrule{2-3} \cmidrule{5-6}
            & Baseline & SDRO (Ours) && Baseline & SDRO (Ours) \\
                
        \midrule 
        LXMERT & 56.92 & 61.53 && 49.47 & 56.18 \\
        UNITER & 63.75 & 63.92 && 57.44 & 58.28 \\
        VILLA  & 64.55 & 63.28 && 58.91 & 57.23 \\
        \bottomrule
    \end{tabular}
    % }
    \caption{Performance on the NLVR$^2$ contrast-set from~\cite{gardner2020evaluating}, which is a manually crafted set of test samples }
    \label{tab:contrast_sets}
\end{table}
